Service Discovery for Hyperledger Fabric

Hyperledger Fabric (HLF) is a modular and extensible permissioned blockchain platform released to open-source and hosted by the Linux Foundation. The platform's design exhibits principles required by enterprise grade business applications like supply-chains, financial transactions, asset management, food safety, and many more. For that end HLF introduces several innovations, two of which are smart contracts in general purpose languages (\emph{chaincode} in HLF), and flexible endorsement policies, which govern whether a transaction is considered valid. Typical blockchain applications are comprised of two tiers: the first tier focuses on the modelling of the data schema and embedding of business rules into the blockchain by means of smart contracts (\emph{chaincode}) and endorsment policies; and the second tier uses the SDK (Software Development Kit) provided by HLF to implement client side application logic. However there is a gap between the two tiers that hinders the rapid adoption of changes in the chaincode and endorsement policies within the client SDK. Currently, the chaincode location and endorsement policies are statically configured into the client SDK. This limits the reliability and availability of the client in the event of changes in the platform, and makes the platform more difficult to use. In this work we address and bridge the gap by describing the design and implementation of \emph{Service Discovery}. \emph{Service Discovery} provides APIs which allow dynamic discovery of the configuration required for the client SDK to interact with the platform, alleviating the client from the burden of maintaining it. This enables the client to rapidly adapt to changes in the platform, thus significantly improving the reliability of the application layer. It also makes the HLF platform more consumable, simplifying the job of creating blockchain applications.

==> endorsement.tex <==
\section{Endorsement Policies}

An endorsement policy is represented in a structure that is called a "signature policy". Before we understand what a signature policy means, lets describe how endorsement policies are validated. In Hyperledger Fabric, policy evaluation can be thought of as a function:
\[
    f := P(identity)\times P(Signature) \leftarrow \{0, 1\}
\]

Informally - the function takes as input a set of identities, and a set of signatures, and either accepts or rejects. The computation of the policy evaluation is comprised of 2 parts:
\begin{enumerate}
    \item	The policy evaluation determines whether the signatures correspond to identities that are privileged to endorse the transaction. The privilege to endorse the transaction is denoted as a set of Principals.  Each identity can satisfy at least some principal, and usually identities of peers satisfy at most one principal, which is their organisational association. There can be several sets of principals that each on its own is deemed sufficient to make the transaction be accepted by the policy evaluation.
    \item	The signatures are verified with their corresponding public keys found in the identities.
\end{enumerate}

Therefore, the endorsement policy itself (what step (1) is evaluating) can be described as a set of sets of principals, such that if the endorsement contains in it signatures that are validated under identities which satisfy some set of principals - the endorsement policy accepts the signatures and the identities, and otherwise - rejects.

An endorsement policy is comprised of 2 objects:
\begin{itemize}
    \item  $P$ - An array of Principals 
    \item  $T$ - A tree that represents the principal sets that the policy expects at least one of them to be satisfied by the identities. The tree has 2 types of vertices:
    \begin{itemize}
        \item Inner vertices (non-leaves) are quantifiers (NoutOf). Each such a vertex specifies how many of its direct descendants should be satisfied for itself to be satisfied.
        \item Leaf vertices are pointers to the array of principals .    
    \end{itemize}
\end{itemize}
Even though quantifiers can denote any number from 1 to the out degree of a vertex, two common use cases are 1OutOf and NoutOf which represent OR and AND respectively. 


\subsection{Endorsement policy evaluation for service discovery}
In the discovery service, an endorsement policy is evaluated to produce combinations of principals such that every combination satisfies the endorsement policy on its own. To compute the combinations of principals, the policy tree $T$ is traversed and sub-trees of $T$ are computed such that the leaf level in every such sub-tree of $T$ is a combination of principals that satisfies the policy. This is done by computing for each inner vertex with an \emph{NoutOf} quantifier of $n$ , all permutations of its descendants of size $n$. Afterwards, the tree $T$ is traversed in BFS and for each inner vertex, the sub-tree is duplicated to accommodate all permutations, until all the vertices are visited.

Having the sub-trees that each sub-tree's leaves are principals that satisfy the endorsement policy, the leaves are aggregated into a histogram that produces a mapping from principals to their plurality in the leaves of the sub-tree. Each such a mapping is a combination of principals and is called a "layout".  The pluralities are used for endorsement policies that require multiple signatures of the same principal, i.e. 3 different identities that correspond to organisation A need to sign, etc.

Aside from layouts, the discovery service computes a mapping from principals to peers. This is done by creating a bi-partite graph $G=(V_1\cup V_2, E)$:
\[
    V_1 := \{ principals \in T\}, V_2 := \{ peers \}, E := \{(u, v) | u \text{ satisfies } v\}
\]
Finally, for each principal  we take all the peers that are connected to it in  to produce a mapping from principals to sets of peers.
This information is then package into an object called an EndorsementDescriptor, which contains information about which peers can be used to request endorsement from, such that the endorsement policy would be fulfilled. 

It contains 2 objects:
\begin{itemize}
   \item Endorsers by groups: maps principals to sets of peers
   \item Layouts: mappings of principals to their needed quantities.
\end{itemize} 

Given an EndorsementDescriptor, clients can compute which peers they should ask for endorsements for using the following algorithm:

\begin{enumerate}
 \item Let $e: G \leftarrow P$ be the "endorsers by groups" field that maps a group to a set of peers
 
 \emph{ Note that applying e on a group g yields a set of peers}.
 \item Select a layout $l: G \leftarrow N$  out of the layouts given. $l$ maps a set of principals to integers which represents amount of peers to select in order for the endorsement policy to be satisfied by the selected layout $l$.
 \item $R := \emptyset$ 
 \item For each group $g \in l$, compute $n=l(g)$  
     \begin{enumerate}
         \item Denote $P_g$ as a set of $n$ random peers $\{p_1, p_2, \dots p_n\}$ selected from $e(g)$.
         \item $R := R \cup P_g$   
     \end{enumerate}
     
 \item The set of peers  is the peers the client needs to request endorsements from.
\end{enumerate}

Note: This selection doesn't take into account network level information which would result in a more appropriate selection of peers, such as - preferring peers with higher ledger heights than other peers, or excluding peers that are found to be offline by the client, etc.

